MedHallu: A Comprehensive Benchmark for Detecting Medical Hallucinations in Large Language Models

Advancements in Large Language Models (LLMs) and their increasing use in medical question-answering necessitate rigorous evaluation of their reliability. A critical challenge lies in hallucination, where models generate plausible yet factually incorrect outputs. In the medical domain, this poses serious risks to patient safety and clinical decision-making. To address this, we introduce MedHallu, the first benchmark specifically designed for medical hallucination detection. MedHallu comprises 10,000 high-quality question-answer pairs derived from PubMedQA, with hallucinated answers systematically generated through a controlled pipeline. Our experiments show that state-of-the-art LLMs, including GPT-4o, Llama-3.1, and the medically fine-tuned UltraMedical, struggle with this binary hallucination detection task, with the best model achieving an F1 score as low as 0.625 for detecting "hard" category hallucinations. Using bidirectional entailment clustering, we show that harder-to-detect hallucinations are semantically closer to ground truth. Through experiments, we also show incorporating domain-specific knowledge and introducing a "not sure" category as one of the answer categories improves the precision and F1 scores by up to 38% relative to baselines.

==> figures/Datapoint_example.tex <==
\begin{table}[h]
    \centering
    \small
    \renewcommand{\arraystretch}{1.2}  % Increases row spacing
    \begin{tabular}{|>{\raggedright\arraybackslash}p{0.1\textwidth}|>{\raggedright\arraybackslash}p{0.3\textwidth}|}
        \hline
        \rowcolor{gray!10} \textbf{Component} & \textbf{Content} \\
        \hline
        \textit{Question} & Is halofantrine ototoxic? \\
        \hline
        \textit{Ground Truth} & Halofantrine has mild to moderate pathological effects on cochlea histology, can be considered ototoxic drug. \\
        \hline
        \textit{Hallucinated Answer} & Halofantrine exhibits no ototoxicity and is generally considered safe for auditory function. \\
        \hline
    \end{tabular}
    \caption{An example in the MedHallu dataset.}
    \label{tab:dataset-example}
\end{table}

==> gemma_results_basic/w_knowledge.tex <==
\begin{table}[h]
\footnotesize  % Make the table smaller
\centering
\setlength{\tabcolsep}{4pt}  % Reduce column spacing
\begin{tabular}{l|c|ccc|c}
\hline
\textbf{Model} & \textbf{Overall} & \textbf{Easy} & \textbf{Med} & \textbf{Hard} & $\Delta$ \\
& \textbf{F1} & \textbf{F1} & \textbf{F1} & \textbf{F1} & \textbf{F1} \\
\hline
GPT-4o mini & \textbf{0.83} & 0.94 & 0.85 & 0.76 & +0.26 \\
Qwen2.5-14B & 0.84 & 0.91 & 0.90 & 0.77 & +0.26 \\
Gemma-9B & 0.82 & 0.92 & 0.87 & 0.76 & +0.23 \\
Qwen2.5-7B & 0.81 & 0.89 & 0.85 & 0.74 & +0.29 \\
Gemma-2B & 0.63 & 0.72 & 0.65 & 0.58 & +0.21 \\
Llama-3.1-8B & 0.79 & 0.89 & 0.82 & 0.73 & +0.35 \\
Llama-3.2-3B & 0.64 & 0.72 & 0.71 & 0.56 & +0.28 \\
Qwen2.5-3B & 0.67 & 0.69 & 0.69 & 0.65 & +0.02 \\
\hline
\end{tabular}
\caption{Performance of LLMs with knowledge. $\Delta$ F1 shows the absolute improvement in Overall F1 score compared to no-knowledge setting. Models are sorted by overall F1 score.}
\label{tab:llm_performance_with_2}
\end{table}


==> gemma_results_basic/wo_knowledge.tex <==
\begin{table}[h]
\footnotesize  % Make the table smaller
\centering
\setlength{\tabcolsep}{4pt}  % Reduce column spacing
\begin{tabular}{l|c|ccc}
\hline
\textbf{Model} & \textbf{Overall F1} & \textbf{Easy F1} & \textbf{Med F1} & \textbf{Hard F1} \\
\hline
GPT-4o mini & 0.57 & 0.77 & 0.71 & 0.42 \\
Qwen2.5-14B & 0.58 & 0.82 & 0.63 & 0.45 \\
Gemma-9B & 0.59 & 0.78 & 0.67 & 0.47 \\
Qwen2.5-7B & 0.52 & 0.76 & 0.56 & 0.38 \\
Gemma-2B & 0.42 & 0.47 & 0.43 & 0.39 \\
Llama-3.1-8B & 0.44 & 0.69 & 0.51 & 0.25 \\
Llama-3.2-3B & 0.36 & 0.53 & 0.43 & 0.23 \\
Qwen2.5-3B & 0.65 & 0.70 & 0.67 & 0.62 \\
\hline
\end{tabular}
\caption{Performance of LLMs without knowledge. Models are sorted by overall F1 score.
\junyuan{What is the main finding in one sentence? You can highlight the best scores in bold.}}
\label{tab:llm_performance_without_2}
\end{table}

==> llama_results_basic/result_table-wo_knowledge.tex <==
\begin{table}[h]
\footnotesize  % Make the table smaller
\centering
\setlength{\tabcolsep}{4pt}  % Reduce column spacing
\begin{tabular}{l|ccc|ccc}
\hline
\textbf{Model} & \textbf{Ove} & \textbf{Overall} & \textbf{Overall} & \textbf{Easy} & \textbf{Med} & \textbf{Hard} \\
& \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{F1} & \textbf{F1} \\
\hline
GPT-4o-mini & 0.71 & 0.86 & 0.61 & 0.82 & 0.72 & 0.60 \\
Qwen2.5-14B & 0.69 & 0.80 & 0.61 & 0.81 & 0.72 & 0.55 \\
GEMMA-9B & 0.68 & 0.79 & 0.61 & 0.81 & 0.70 & 0.53 \\
Qwen2.5-7B & 0.64 & 0.76 & 0.55 & 0.70 & 0.71 & 0.51 \\
DeepSeek-8B & 0.61 & 0.68 & 0.55 & 0.68 & 0.61 & 0.54 \\
\hline
\end{tabular}
\caption{Performance of LLMs without knowledge. Overall F1/P/R represents metrics computed on the entire dataset. Models are sorted by overall F1 score.}
\label{tab:llm_performance_without}
\end{table}

==> llama_results_basic/result_table_merged.tex <==
\begin{table*}
\centering
\begin{tabular}{l|ccc|ccc|c|c}
\hline
\textbf{Model} & \textbf{Overall F1} & \textbf{Overall Pr} & \textbf{Overall Re} & \textbf{Easy F1} & \textbf{Med F1} & \textbf{Hard F1} & $\Delta$ \textbf{Know.} & \textbf{Avg} \\
\hline
Qwen2.5-14B \\
~~w/o knowledge & 0.69 & 0.80 & 0.61 & 0.81 & 0.72 & 0.55 & - & 0.70 \\
~~w/ knowledge & \textbf{0.86} & 0.85 & 0.87 & 0.89 & 0.87 & 0.82 & +0.17 & 0.86 \\
\hline
GPT-4o-mini \\
~~w/o knowledge & 0.71 & 0.86 & 0.61 & 0.82 & 0.72 & 0.60 & - & 0.72 \\
~~w/ knowledge & 0.85 & 0.85 & 0.85 & 0.91 & 0.86 & 0.77 & +0.14 & 0.85 \\
\hline
Qwen2.5-7B \\
~~w/o knowledge & 0.64 & 0.76 & 0.55 & 0.70 & 0.71 & 0.51 & - & 0.65 \\
~~w/ knowledge & 0.85 & 0.84 & 0.85 & 0.92 & 0.87 & 0.77 & +0.21 & 0.85 \\
\hline
GEMMA-9B \\
~~w/o knowledge & 0.68 & 0.79 & 0.61 & 0.81 & 0.70 & 0.53 & - & 0.69 \\
~~w/ knowledge & 0.82 & 0.78 & 0.86 & 0.86 & 0.82 & 0.78 & +0.14 & 0.82 \\
\hline
DeepSeek-8B \\
~~w/o knowledge & 0.61 & 0.68 & 0.55 & 0.68 & 0.61 & 0.54 & - & 0.61 \\
~~w/ knowledge & 0.82 & 0.86 & 0.79 & 0.84 & 0.85 & 0.77 & +0.21 & 0.82 \\
\hline
\end{tabular}
\caption{Performance comparison of different LLMs with and without knowledge. Overall F1/P/R represents metrics computed on the entire dataset. $\Delta$ Knowledge shows the average absolute improvement across all metrics when knowledge is provided. The rightmost column shows the average of all metrics per model condition. All values are rounded to 2 decimal places. Models are sorted by overall F1 score with knowledge.}
\label{tab:llm_performance}
\end{table*}

==> llama_results_basic/result_table_w-knowledge.tex <==
\begin{table}[h]
\footnotesize  % Make the table smaller
\centering
\setlength{\tabcolsep}{4pt}  % Reduce column spacing
\begin{tabular}{l|c|ccc|c}
\hline
\textbf{Model} & \textbf{Overall} & \textbf{Easy} & \textbf{Med} & \textbf{Hard} & $\Delta$ \\
& \textbf{F1} & \textbf{F1} & \textbf{F1} & \textbf{F1} & \textbf{F1} \\
\hline
Qwen2.5-14B & \textbf{0.86} & 0.89 & 0.87 & 0.82 & +0.17 \\
GPT-4o-mini & 0.85 & 0.91 & 0.86 & 0.77 & +0.14 \\
Qwen2.5-7B & 0.85 & 0.92 & 0.87 & 0.77 & +0.21 \\
GEMMA-9B & 0.82 & 0.86 & 0.82 & 0.78 & +0.14 \\
DeepSeek-8B & 0.82 & 0.84 & 0.85 & 0.77 & +0.21 \\
\hline
\end{tabular}
\caption{Performance of LLMs with knowledge. $\Delta$ F1 shows the absolute improvement in Overall F1 score compared to no-knowledge setting. Models are sorted by overall F1 score.}
\label{tab:llm_performance_with}
\end{table}
